Persistent Negatives for Adversarial Black-Box On-Policy Distillation

Black-box On-Policy Distillation (OPD) seeks to improve a student from its own generations when the teacher provides sampled responses but not token probabilities. Adversarial distillation offers one route: it learns a discriminator over prompt-matched teacher and student responses and uses its score as the policy reward. However, sampling discriminator negatives from the latest student at each step couples the learned reward to a negative distribution that changes after every policy update. We address this moving-target problem with persistent-negative adversarial distillation, a live-pool method that replaces a fraction of each discriminator batch with historical, prompt-matched teacher--student comparisons. Under matched discriminator compute, historical comparisons train the discriminator, while GRPO remains on-policy with fresh student responses. Our analysis identifies the Bayes-optimal reward as a teacher-to-negative log-density ratio and, under explicit assumptions, shows how persistent negatives anchor the discriminator and reduce reward-estimation MSE relative to fresh-negative training. Across two student families, three judges, and four judged-chat benchmarks, persistent-negative adversarial distillation consistently improves performance over current methods at matched discriminator compute. It also yields smoother fresh-policy discriminator trajectories, with fewer below-chance dips. These findings identify the discriminator's negative distribution as an important design axis in black-box on-policy distillation.

==> Makefile <==
main.pdf: main.tex \
	iclr2027_conference.sty \
	iclr2027_conference.bst \
	natbib.sty \
	fancyhdr.sty \
	shared/abstract.tex \
	shared/body.tex \
	shared/appendix.tex \
	shared/macros.tex \
	refs.bib \
	figures/intro_live_pool_gad.pdf \
	figures/pool_setup_comparison.pdf \
	figures/judged_chat_paired_effects.pdf
	pdflatex -interaction=nonstopmode -halt-on-error main.tex
	bibtex main
	pdflatex -interaction=nonstopmode -halt-on-error main.tex
	pdflatex -interaction=nonstopmode -halt-on-error main.tex

clean:
	rm -f main.aux main.bbl main.blg main.log main.out main.toc main.fls main.fdb_latexmk main.synctex.gz missfont.log

distclean: clean
	rm -f main.pdf

.PHONY: clean distclean

